Efficient Geometry-aware 3D Generative Adversarial Networks

Unsupervised generation of high-quality multi-view-consistent images and 3D shapes using only collections of single-view 2D photographs has been a long-standing challenge. Existing 3D GANs are either compute-intensive or make approximations that are not 3D-consistent; the former limits quality and resolution of the generated images and the latter adversely affects multi-view consistency and shape quality. In this work, we improve the computational efficiency and image quality of 3D GANs without overly relying on these approximations. We introduce an expressive hybrid explicit-implicit network architecture that, together with other design choices, synthesizes not only high-resolution multi-view-consistent images in real time but also produces high-quality 3D geometry. By decoupling feature generation and neural rendering, our framework is able to leverage state-of-the-art 2D CNN generators, such as StyleGAN2, and inherit their efficiency and expressiveness. We demonstrate state-of-the-art 3D-aware synthesis with FFHQ and AFHQ Cats, among other experiments.

==> disabled/supplement_wrapper.tex <==
%%%%%%%%%% Merge with supplemental materials %%%%%%%%%%
\pagebreak
\widetext
\begin{center}
\textbf{\large Supplemental Material\\Efficient Geometry-aware 3D Generative Adversarial Networks}
\end{center}

%%%%%%%%%% Merge with supplemental materials %%%%%%%%%%
%%%%%%%%%% Prefix a "S" to all equations, figures, tables and reset the counter %%%%%%%%%%
\setcounter{equation}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{page}{1}
\makeatletter
\renewcommand{\theequation}{S\arabic{equation}}
\renewcommand{\thefigure}{S\arabic{figure}}
\renewcommand{\bibnumfmt}[1]{[S#1]}
\renewcommand{\citenumfont}[1]{S#1}
%%%%%%%%%% Prefix a "S" to all equations, figures, tables and reset the counter %%%%%%%%%%


In this supplement, we first provide additional experiments (Section~\ref{sec:supp_additional_experiments}) and visual results (Section~\ref{sec:supp_additional_visual_results}). We follow with details of our implementation (Section~\ref{sec:supp_implementation_details}), including further descriptions of model architecture and training process, as well as hyperparameters. We discuss experiment details (Section~\ref{sec:supp_experiment_details}), such as datasets and baselines, and further explanations for experiments such as inversion. Lastly, we consider artifacts (Section~\ref{sec:supp_discussion}) that may be targets of future work. We encourage readers to view the accompanying supplemental video, which contains additional visual results, including a live demonstration of real-time synthesis.


\input{sections/supplemental/additional_experiments}


\input{sections/supplemental/additional_visual_results}

\input{sections/supplemental/implementation_and_experiment_details}

\input{sections/supplemental/supplemental_discussion}

%%%%%%%%% REFERENCES
\clearpage

{\small
\bibliographystyle{ieee_fullname}
\bibliography{egbib}
}


==> sections/3d_representation_and_rendering.tex <==
%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\linewidth]{images/pipeline2}
%    \caption{Illustration of network architecture. We leverage a StyleGAN2 generator, including the modulation weights $w$ (A) created by a mapping network (B) that is conditioned on a latent code $z$ and the camera pose $Rt,K$. The generator outputs three channels, which are reshaped (C) into axis-aligned feature planes $F_p$ (D). A neural volume rendering step integrates many 3D samples of the feature volume along each ray to project it into a 2D feature image $F_{\textrm{NR}}$ (E). The neurally rendered features are upsampled by a CNN-based super-resolution module (F) then concatenated to the upsampled neural rendered output (G) before being fed into a StyleGAN2 discriminator, which is conditioned on the camera pose via another mapping network (H).}
%    \label{fig:pipeline}
%\end{figure}
\kn{Since we are selling the efficiency primarily, I think it's critical to report the run-time comparison of representation itself to MipNeRF, NSVF, and Cube.}\gw{absolutely! the problem is that our tri-plane rep in this experiment is much larger than the tri-plane rep used in our GAN. the former isn't much faster than nerf whereas the latter is. }\kn{lets show both and say the GAN one is our main and practical config!}
Training a high-resolution GAN requires a 3D representation that is both efficient and expressive. In this section, we introduce a new hybrid explicit--implicit tri-plane representations that offer both of these advantages. We introduce the representation in this section using a single-scene overfitting scenario, before discussing how it is integrated in our GAN framework in the next section.

%\jt{we could possibly consider a better link from the previous section to this one then something about a limitation}. 
%As discussed, the inefficiency of MLP-based volume rendering hinders native rendering at high resolutions; this puts a limit on image quality, or if convolutional upsampling layers are used, on shape quality and view-consistency. Inspired by recent hybrid explicit--implicit 3D representations that combine explicit features with an implicit decoder, we introduce a tri-plane-based hybrid 3D representation to achieve both efficient and expressive 3D-aware image synthesis. 

% \begin{equation}
%     F_{planes}, w = G_{B}(z, Rt, K)
% \end{equation}

% We use an off-the-shelf CNN backbone to generate a $256 \times 256 \times 96$ feature image, which is reshaped into three orthogonal 32-channel feature planes that span the volume. 

In the tri-plane formulation, we align our explicit features along three axis-aligned orthogonal feature planes, each with a resolution of $N \times N \times C$ (Figure. \ref{fig:hybrid_representation}c) with $N$ being a spatial resolution and $C$ a number of channels. Any 3D point $x \in \mathbb{R}^3$ can be queried by projecting $x$ onto each of the three feature planes, retrieving the corresponding feature vector via bilinear interpolation, and aggregating the three feature vectors via summation. An additional lightweight decoder network, implemented as a small MLP, interprets the aggregated 3D features as color and density. These quantities are rendered into RGB images using (neural) volume rendering~\cite{Max:1995,mildenhall2020nerf}. 

\begin{figure}[t!]
	\centering
		\includegraphics[width=\columnwidth]{images/overfitting.png}		
		\caption{Multi-view reconstruction of a Tanks \& Temples~\cite{Knapitsch2017} scene with 152 images. A fully implicit NeRF (left) and a dense voxel grid representation (center right) do not capture detail, such as the text. Neural sparse voxel fields (NSVF) allocate voxel resolution adaptively (center left). The proposed tri-plane representation with the same number of features as the feature cube captures the most detail (right). 
% 		\jt{I am happy to also add the LPIPS metrics if you send me the images. Reviewers might be saying this is anecdotal results, do we have more results on more scenes, e.g., the synthetic nerf scenes? } \cl{I think we should be good with PSNR and SSIM since this is mostly a small proof of concept figure? We don't have results on other scenes, but this scene is pretty detailed and maybe we can run other scenes for the appendix.}
		}
		\label{fig:overfitting}
\end{figure}

\begin{table}
\centering
		\small
    \begin{tabular}{l c c c}
\toprule
               & MLP & Rel. Speed $\uparrow$ & Rel. Mem. $\downarrow$   \\ 
%\cline{1-3}
        \midrule
Fully Implicit &$8\times256$      & $1\times$         & $1\times$ \\
w/ Voxels &$4\times128$   & $3.5\times$       & $0.33\times$ \\
w/ Tri-plane (SS) &$4\times128$ & $2.9\times$       & $0.32\times$  \\
w/ Tri-plane (GAN) &$1\times64$  & $7.8\times$       & $0.06\times$  \\
\bottomrule
\end{tabular}
\caption{Hybrid representations with small implicit decoders are faster and less memory intensive than large MLPs of similar capability. \# hidden layers and \# hidden units of the MLP are specified. Tri-plane (GAN) forms the heart of our GAN framework (Section~\ref{sec:gan_framework}) and is much lighter weight than the one used in the single-scene (SS) evaluation.}
\label{tab:overfitting_speed}
\end{table}

By keeping the decoder small and shifting the bulk of network capacity into the explicit plane features, we reduce the computational cost of neural rendering by a factor of 2--10$\times$ compared to similar implicit MLP architectures~\cite{chan2020pi}. Such an improvement accelerates training and allows for native rendering at higher resolutions, a necessary component for generating high-quality view-consistent images and detailed shapes.

%By keeping the decoder small and shifting the bulk of network capacity into the explicit plane features, we reduce the computational cost of neural rendering by nearly an order-of-magnitude versus a comparable MLP~\cite{chan2020pi}\ec{I think we need to be careful in discussing performance numbers in this section because the model for single-scenes and for generalization are different— our single-scene model is 4 layers of 128 and is about 2-2.5x faster than NeRF/pi-GAN; our generalization model is 1 layer of 64 and is about 7-10x faster than NeRF/pi-GAN.}. Such an improvement accelerates training and allows for native rendering at higher resolutions, a necessary component for generating view-consistent images and detailed shapes.




\begin{figure*}[t]
	\footnotesize
	\centering
	\includegraphics[width=\linewidth]{images/pipeline.pdf}
	\caption{3D GAN pipeline.\og{triplane $\rightarrow$ tri-plane}
% 	\kn{Change renderer to decoder. the figure needs to show the RAW image is the first 3 channels of the feature image from the deocder. Add volume rendering between decoder and the feature image. check camera param numbers. Add proper symbols used in text. Also it helps to add how many channel features goes into the MLP decoder in Figure 4}
	}
	\label{fig:pipeline}
\end{figure*}

% \begin{figure*}[t]
% 	\footnotesize
% 	\centering
% 	\includegraphics[width=\linewidth]{images/line_drawing_2.png}
% 	\caption{3D GAN pipeline.
% % 	\kn{Change renderer to decoder. the figure needs to show the RAW image is the first 3 channels of the feature image from the deocder. Add volume rendering between decoder and the feature image. check camera param numbers. Add proper symbols used in text. Also it helps to add how many channel features goes into the MLP decoder in Figure 4}
% 	}
% 	\label{fig:pipeline}
% \end{figure*}

% \ec{The tri-plane and cube models have comparable number of embeddings but both have far more than NSVF in this experiment, since NSVF can prune empty voxels. Perhaps we should instead specify that computation cost (in terms of runtime/memory per sample) is comparable?}

% Because it is not intuitive that a tri-plane representation would be able to adequately capture complex scenes, we evaluate the representation with a common novel-view synthesis setup, i.e., we directly optimize the features of the planes and the weights of the decoder to fit $360^\circ$ views of a scene from the tanks \& temples dataset~\cite{Knapitsch2017}.
To validate the tri-plane representation is compact yet offers sufficient expressiveness, we evaluate the representation with a common novel-view synthesis setup, i.e., we directly optimize the features of the planes and the weights of the decoder to fit $360^\circ$ views of a scene from the tanks \& temples dataset~\cite{Knapitsch2017} (Figure~\ref{fig:overfitting}).
% \og{``not intuitive'' may sound negative. How about ``To validate that a representation as compact as our tri-plane offers sufficient expressiveness...''} 
%, a common novel-view synthesis setup~\cite{mildenhall2020nerf} \kn{say which dataset (tanks \& temples? just 1 scene or are we reporting more in appendix?) commonly used in this task}. 
% Figure~\ref{fig:overfitting} shows the results of this experiment.
In this demonstration, we use feature planes of resolution $N=512$ and channels $C=48$, paired with an MLP of four layers of 128 hidden units; we compare the results against a dense feature volume of equal capacity. For reference, we include comparisons to a fully implicit 3D representation~\cite{barron2021mipnerf} and neural sparse voxel fields (NSVF)~\cite{liu2020neural}. Figure~\ref{fig:overfitting} demonstrates that the tri-plane representation is capable of fitting to this complex scene, outperforming dense feature volume representations~\cite{sitzmann2019deepvoxels,Lombardi:2019} and fully implicit representations~\cite{mildenhall2020nerf} while performing competitively with NSVF~\cite{liu2020neural}. For simplicity, we do not include view-dependent effects.
% \kn{Can we also report run-time performance here?}
\ec{comment on view-dependent effects}
\ec{Mention that NSVF cannot be used easily in generalization}
Moreover, in keeping the decoder small, we achieve a $2 \times$ speed-up compared to an 8-layer MLP.
% — in section ~\ref{sec:gan_framework} we further reduce the size of the decoder to a single hidden layer of 64 units, which pushes the speed-up to $7 \times$.
\ec{Potentially report performance, but run risk of confusing reader between single-scene and GAN settings}\kn{Show the run-time comparison of (1) our representation using the same capacity as other baselines along with their runtime (2) also report a run-time of GAN setting and say that with the CNN, we can practically operate at much faster speed by combining a CNN backbone and describe the reduced setting in the next section.}
\ec{Potentially report memory constraints as well}


% The tri-plane architecture's simplicity and efficiency makes it an attractive option for our 3D-aware GAN application, where rendering speed during training is paramount. In the following sections, we adapt the tri-plane representation for generalization across scenes by predicting the feature planes with a high-capacity 2D CNN backbone.

The tri-plane architecture is more memory-efficient than voxel grids and faster than MLPs of comparable quality. Additionally, unlike MLPs, voxels, or trees, the tri-plane representation is simple to interface with powerful off-the-shelf 2D CNN backbones, a pairing which we describe in the following sections.

% \ec{I think we need to stress that another advantage of tri-planes over trees \& volumes is that it interfaces simply with 2D CNN's. We can discuss that either here or later on.} \sg{This is a good point. We haven't discussed the tree-based optimizations of Nerf at all...}
% \og{I agree that we need to discuss the fact that tri-planes allow to work with 2D CNNs, and I think that here is the right place.}

% Keep the discussion like below in the Intro, Related work or Colclusion, not in the Method section
%To our knowledge, this is the first such tri-plane hybrid architecture used for 3D GANs, although a combination of feature volumes or locally conditioned implicit functions have been used in other variants~\cite{devries2021unconstrained} or for other applications~\cite{peng2020convolutional} in the past. The neural rendering community at large may be interested in the same benefits for other applications.




% The tri-plane architecture's  simplicity, generalizability, expressiveness, computational efficiency, and flexibility to interface with any 2D CNN backbone makes the tri-plane representation ideal for our 3D GAN application. To our knowledge, this is the first such hybrid architecture used for 3D GANs, although a combination of feature volumes or locally conditioned implicit functions have been used in other variants~\cite{devries2021unconstrained} or for other applications~\cite{peng2020convolutional} in the past. The neural rendering community at large may be interested in the same benefits for other applications.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/methods.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/pipeline2}
    \caption{Illustration of network architecture. We leverage a StyleGAN2 generator, including the modulation weights $w$ (A) created by a mapping network (B) that is conditioned on a latent code $z$ and the camera pose $Rt,K$. The generator outputs three channels, which are reshaped (C) into axis-aligned feature planes $F_p$ (D). A neural volume rendering step integrates many 3D samples of the feature volume along each ray to project it into a 2D feature image $F_{\textrm{NR}}$ (E). The neurally rendered features are upsampled by a CNN-based super-resolution module (F) then concatenated to the upsampled neural rendered output (G) before being fed into a StyleGAN2 discriminator, which is conditioned on the camera pose via another mapping network (H).}
    \label{fig:pipeline}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The architecture of our 3D GAN comprises of five major parts: a 2D CNN-based feature plane generator network, two mapping networks, a neural volume rendering engine, a 2D CNN-based image upsampling network, and a discriminator. This pipeline is illustrated in Fig.~\ref{fig:pipeline} and designed with two goals in mind: expressiveness and computational efficiency. The former is important for synthesizing diverse, photorealistic, and multi-view consistent scenes. Efficiency is equally crucial for training a 3D GAN on large-scale image datasets, which typically requires tens or hundreds of millions of feedforward network queries. Although this is computationally infeasible for most prior approaches, neural rendering remains an essential part of our 3D GAN as it adds the inductive bias necessary for geometry-aware 3D image synthesis. 

Instead of designing a generator network from scratch, we adapt StyleGAN2's generator architecture with subtle but important modifications, including its mapping network~\cite{Karras2020stylegan2}. This choice is motivated by the fact that StyleGAN2 is a well-understood, flexible, and efficient architecture that achieves state-of-the-art results for 2D image synthesis. However, it lacks an inductive bias for multi-view consistent and geometry-aware 3D synthesis, which our framework aims to remedy. Our generator outputs three axis-aligned neural feature planes in Euclidean space to form a feature volume (D) in Fig. \ref{fig:pipeline}. This volume can be projected into 2D images using neural volume rendering~\cite{mildenhall2020nerf}. Due to the computational cost of this last step, we render at a moderate resolution and follow~\cite{Niemeyer2020GIRAFFE} in applying a CNN-based image upsampling network. The result is fed into a discriminator which again builds strongly on the StyleGAN2 architecture, but adds camera pose conditioning and a dual discrimination strategy to promote multi-view consistency. In the following subsections, we describe the novel parts of our architecture. For additional details on StyleGAN2 or neural volume rendering, we refer to the original works introducing those methods. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% GW: I commented this out because related work should be primarily discussed in the related work section and not here.

%\subsection{Image Synthesis with 3D-Aware GANs}
%
%Like previous 3D-Aware GANs\cite{graf}\cite{chan2020pi}\cite{Niemeyer2020GIRAFFE}, we take advantage of adversarial training to indirectly learn 3D representations. Rather than directly generating 2D images from input noise as in traditional 2D image GANs, 3D-Aware generators produce a 3D representation conditioned on the input noise that is then rendered into a 2D image from an input rendering view. At training time, synthesized 2D renderings as well as real 2D images from the dataset are directed to a traditional convolutional discriminator for adversarial training. At inference, a 3D-Aware generator can decouple identity and camera viewpoint to enable viewpoint-controllable image synthesis and the latent 3D representations can be leveraged for downstream tasks.
%
%Although 3D-Aware generative models have demonstrated impressive results, the computational cost of view-consistent neural rendering continues to be a bottleneck. Because typical volumetric rendering approaches, like NeRF\cite{mildenhall2020nerf}, take several seconds to render even moderately sized images, inference at real-time framerates becomes a challenge. Even more importantly, since the training process of 3D-Aware GANs requires rendering many millions of images, compute limits have limited image size and model capacity, meaning the quality of 3D-Aware GANs have lagged far behind their 2D counterparts.
%
%Recent methods have approached this computational bottleneck in one of two ways.
%
%\cite{graf} and \cite{chan2020pi} have stuck to 3D-grounded volumetric rendering, which enables enables image synthesis with high multi-view consistency and high-quality intermediate shape representations. However, the computational expense of volumetric rendering places a limit on both the quality of images as well as the speed of training and inference.
%
%\cite{hologan} and \cite{Niemeyer2020GIRAFFE} instead perform 3D-grounded rendering at low resolutions and rely primarily on image-space convolutional and upsampling layers to enlarge and refine the image output. Such methods obtain high-quality images efficiently, but since image-space convolutions are not naturally 3D consistent, these methods suffer from worse multi-view consistency and low-quality intermediate shapes.
%
%In our approach, we take a third track. Drawing inspiration from recent hybrid approaches\cite{martel2021acorn} that combine an explicit backbone with a lightweight implicit ``decoder", we significantly improve the computational efficiency of the implicit model. Such dramatic reductions in memory and computation time enable volumetric rendering at higher resolutions than previous approaches, giving our approach the capability of generating larger images than 3D-grounded methods without sacrificing view-consistency or high-quality shapes. We augment the raw neural renderings with an image-space ``superresolution" module that enhances and enlarges the raw output of volumetric rendering but we introduce ``dual-discrimination" as a means to ensure consistency between the raw neural rendering and the superresolution output, which prevents the worst effects of view inconsistency. Our combined pipeline enables image synthesis of large, high-quality images while also maintaining strong view-consistency and learning high-fidelity intermediate 3D shapes.


% The general training strategy of 3D-Aware GANs is well proven, with each successive method improving on the last.

% General training Strategy for 3D-Aware GAN

% Volume Rendering

% Identify the primary shortcoming of previously proposed 3d-aware GANs:
% Computational efficiency

\subsection{Tri-plane Volume Representation}
%  [Triplane Hybrid Explicit-Implicit Volume Representation]

Neural volume rendering requires a 3D scene representation produced by the network generator. To achieve this goal, we propose a hybrid explicit--implicit strategy that uses StyleGAN2 to generate three orthogonal feature planes, which span the volume. Any 3D point $x \in \mathbb{R}^3$ can be queried by projecting $x$ on each of the three feature planes, retrieving the corresponding feature vector $f_i$ via bilinear interpolation, and aggregating the three feature vectors via summation. An additional lightweight decoder network (i.e., a multilayer perceptron with one hidden layer) converts 3D features into color $\mathbf{c}(x)$ and density $\sigma(x)$. These quantities are rendered into 2D images using (neural) volume rendering~\cite{Max:1995,mildenhall2020nerf}. 

%The pixel color $\mathbf{C}$ for a camera ray $\mathbf{r}(t) = \mathbf{o} + t \dir$ with near and far bounds $t_n$ and $t_f$ is then calculated using the volume rendering equation~\cite{Max:1995}:
%
%\begin{align}
%\label{eqn:volumetric_rendering}
%\begin{split}
    %\mathbf{C} (\mathbf{r}) & = \int_{t_n}^{t_f} T(t) \density \left(\mathbf{r}(t) \right) \col \left(\mathbf{r}(t),\dir \right)dt,
%\\
%& \text{where} \quad
%T(t)  = \text{exp} \left(-\int_{t_n}^{t}\sigma(\mathbf{r}(s))ds \right).
%\end{split}
%\end{align}

This tri-plane representation combines the computational efficiency of explicit representations with the continuous and expressive nature of implicit representation. Moreover, it inherits none of their disadvantages, because the tri-plane feature volume is two orders of magnitude more memory efficient than a dense feature volume~\cite{sitzmann2019deepvoxels,Lombardi:2019,chan2020pi} and the lightweight implicit decoder makes it significantly faster to query than the deep MLPs used by many implicit architectures~\cite{mildenhall2020nerf,chan2020pi}. To our knowledge, this is the first such hybrid architecture used for 3D GANs, although a combination of feature volumes or locally conditioned implicit functions have been used in other variants~\cite{devries2021unconstrained} or for other applications~\cite{peng2020convolutional} in the past.

\ec{The tri-plane and cube models have comparable number of embeddings but both have far more than NSVF in this experiment, since NSVF can prune empty voxels. Perhaps we should instead specify that computation cost (in terms of runtime/memory per sample) is comparable?}
Figure~\ref{fig:overfitting} demonstrates that our tri-plane representation is competitive with and, in this experiment, outperforms both an adaptively refined sparse voxel field~\cite{liu2020neural} and also a dense feature volume representation~\cite{sitzmann2019deepvoxels,Lombardi:2019,chan2020pi} for a comparable number of features. This is an ``overfitting'' experiment in which we distill multiple input views of a single scene from the Tanks \& Temples dataset~\cite{Knapitsch2017} into the respective neural scene representation. The tri-plane representation performs remarkably well, as it only stores features on the three axis-aligned planes rather than in the full 3D space. Its expressiveness, low memory footprint, extremely high computational efficiency, and compatibility with 2D CNN-based backbone networks makes the tri-plane representation ideal for our 3D GAN application. The neural rendering community at large may be interested in the same benefits for other applications.

%Key to our approach is an efficient hybrid explicit-implicit architecture that allows 3D-grounded rendering at high resolutions. While most previous hybrid methods have chosen either tree structures\cite{martel2021acorn}\cite{chabra2020deep}, which are efficient but do not lend themselves to generalization, or uniform voxel grids\cite{Lombardi:2019}, which can generalize but don't scale to high resolutions, we choose a set of three orthogonal feature planes to represent the explicit component of our architecture.~\cite{peng2020convolutional}? The triplane formulation provides the computational efficiency benefit of hybrid architectures while being simpler and easier to generalize across than trees, and without suffering cubic resolution scaling of uniform voxel grids. Just as importantly, the triplane representation allows us to leverage the large body of work on 2D convolutional networks— we can use any off-the-shelf 2D convolutional network to generate the feature planes, e.g. image-to-image translation models or 2D image GANs.

%Our hybrid triplane architecture consists of an explicit plane-generation backbone and a single-hidden-layer implicit decoder. For any 3D point $x \in \mathbb{R}^3$, we project orthogonally to each feature plane $p_i$ and retrieve a feature vector $f_i$ via bilinear interpolation. We aggregate feature vectors by summation and pass the aggregated feature vectors to the implicit decoder, which produces density $\sigma(x)$ and rendered features $F_{NR}$.

% Fully implicit representations are inefficient for volumetric rendering, as each ray sample requires an expensive evaluation of a large MLP. Instead, we employ a hybrid explicit-implicit representation consisting of a set of learned 2D feature planes $\{p_i\}$.

% During rendering, we project a ray sample $x \in \mathbb{R}^3$ to each feature plane $p_i$ and obtain feature vectors $f_i$ via bilinear interpolation. These feature vectors are aggregated by summation and passed through a very lightweight single-layer decoder that outputs the predicted color $c(x)$ and density $\sigma(x)$ for volume rendering. 

%Since the feature planes $\{p_i\}$ are efficently generated in a single pass of the backbone and are shared across ray samples, our approach is much more computationally efficient than comparable fully implicit methods. 

%\ec{Probably need more explanation for overfitting experiments}
%Figure 2 demonstrates how our 3-plane representation performs on par or better than both representations.

% Key advantages of 3-plane representation:
% 2D Convolutional Generators

% How it works
% Convolutional network
% Feature aggregation

% Superresolution module

% \begin{itemize}
%     \item motivate and describe this hybrid explicit--implicit representation
%     \item describe sampling via feature aggregation 
%     \item volume rendering
%     \item derive computational efficiency using big-O notation
%     \item show overfitting results right here and comparison against NSVF, Dense Cube, Three-Plane; although neither voxel cube nor planes model specular reflections in this setting
% \end{itemize}

% Notes:
% \begin{itemize}
%     \item Check apple paper~\cite{devries2021unconstrained} - 2D CNN generator for ground plane with features that locally condition NeRF, convolutional occupancy networks~\cite{peng2020convolutional} - features live on plane(s) or grid, processed by CNN and then decoder on top, ACORN - adaptive grid of features with lightweight decoder on top
%     \item Advantages: simple, fast (because small implicit component), generalizable, and easily interfaces with 2D convolutional networks.
% \end{itemize}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Multi-view Consistent Image Super-resolution}

Although our 3D representation network is significantly more efficient than comparable architectures, it is still too slow to train a 3D GAN directly on high-resolution images. To mitigate this challenge, we rely on an image ``super-resolution'' module composed of image-space 2D convolutional layers to upsample and refine the neurally rendered features. To avoid multi-view consistency issues observed in prior work~\cite{hologan,Niemeyer2020GIRAFFE}, we introduce a method to ensure consistency between the super-resolved images and the neurally rendered images: \textit{dual-discrimination}.

To this end, we pass the discriminator not only the super-resolved images, but also the raw neural rendering. Correspondingly, for real images, we pass the discriminator the real image as well as a downsampled copy of the same image. Dual-discrimination has three benefits: it encourages the final super-resolution output to match the distribution of real images; it encourages the neural rendering to match the distribution of downsampled real images; it encourages the super-resolved images to be consistent with the neural rendering. Using dual-discrimination, we can leverage convolutional layers for higher image-quality without suffering from view-inconsistency artifacts. In practice, dual discrimination is straightforward to implement: we upsample the neural rendered images to the same resolution as the super-resolved output and pass the concatenated images to the discriminator as a six channel image input. 

%Our triplane formulation makes the process of volumetric rendering far more palatable than rendering with MLPs— runtime-per-sample is reduced by nearly an order of magnitude. However, even such improvements are not enough to enable scaling to resolutions beyond $256^2$ on conventional hardware. To close the quality and image-size gap with 2D image GANs, we rely on a ``superresolution" module composed of image-space 2D convolutional layers to upsample and refine the neural-rendered features. However, in order to avoid the multi-view-consistency issues that plagued previous methods\cite{hologan}\cite{Niemeyer2020GIRAFFE} that also relied on image-space convolutions, we introduce a method to ensure consistency between the superresolution output and the raw neural-rendered output: \textit{dual-discrimination}.

% \paragraph{Dual-Discrimination.}

% Convolutional layers are well-proven for realistic image synthesis. Compared to pixel-independent neural-rendering, convolutional layers are simple, expressive, and efficient. We rely on several layers of convolutions as an inexpensive way to upsample, de-noise, and refine our neural-rendered output. However, image-space convolutions, while … are not view consistent. Left unregulated, these convolution layers learn viewpoint-inconsistent effects, despite operating on top of viewpoint-consistent neural rendering. We propose dual-discrimination as a method of regulating the convolutional super-resolution layers.

%When discriminating generated images, we pass the discriminator not only the final, super-resolution output, but also the raw, neural-rendered output. Correspondingly, for real images, we pass the discriminator the real-image as well as a downsampled copy of the same image. Dual-discrimination has three effects. It encourages the final, super-resolution output to match the distribution of real images; it encourages the neural-rendered outputs to match the distribution of downsampled real images; it encourages the super-resolution output to be consistent with the neural-rendered output. With dual-discrimination, we are able to take advantage of the image-quality improvements lent by convolutional layers without suffering the view-inconsistency that typically follows them. In practice, dual discrimination is simple to implement: we upsample the raw-neural-rendering to the same size as the superresolution output and pass the concatenated images to the discriminator as a six channel image. In combining dual-discrimination with the already high-resolution rendering afforded by the efficient architecture, our proposed approach effectively scales to large, high-quality images while maintaining a high degree of multi-view consistency.

%\ec{Do we need to define multi-view consistency somewhere?}

%... \ec{Clarify how are we different from other methods? higher neural rendering resolution, dual discrimination}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Learning Pose-correlated Attributes}
\kn{I think pose-correlated attributes might be more general/precise word than "appearance" since we are not explicitly modeling "appearance" and we want to avoid criticism. }
Interestingly, datasets like FFHQ include biases that correlate camera pose and appearance. For example, the camera angle with respect to a person's face plays a significant role in whether the person smiles in a photo (see Figure~\ref{fig:smiliness}). Learning such view-dependent biases is important for achieving the best image quality, but it is difficult to model these using a 3D-aware generator without also introducing inconsistencies. Related work has been successful in being either view consistent~\cite{graf,chan2020pi,shi2021lifting} or able to model pose-appearance correlations~\cite{hologan,Niemeyer2020GIRAFFE} but not both simultaneously. 

We introduce \textit{generator pose conditioning} as a means to model correlations between pose and appearance in the image distributions we use to train our GAN. To this end, we provide the mapping network not only a latent code vector $z$ as input but also the camera pose. During training, pose conditioning allows the generator to learn implicit biases of the network that are pose dependent. To prevent view inconsistent rendering during inference, however, we disable the generator pose conditioning after the GAN is fully trained. Note that always conditioning the generator with the true camera pose can lead to degenerate solutions where the GAN produces 2D billboards angled towards the camera. To prevent these degeneracies, we induce noise to the camera pose during training.

\subsection{Formalizing the Training Setup \textcolor{red}{GW: I think we should omit this subsection}}

We define camera extrinsics $Rt$, camera intrinsics $K$, input noise vector $z$, and generator components $G_{B}$, $G_{R}$, $G_{SR}$ for the backbone, renderer, and superresolution modules respectively.

The generator backbone, in our case based on StyleGAN2, is conditioned on input noise and camera parameters and produces a 96-channel feature image $F_{planes}$ and latent vector $w$ (the output of the mapping network).

\begin{equation}
    F_{planes}, w = G_{B}(z, Rt, K)
\end{equation}

$F_{planes}$ is reshaped into three 32-channel feature planes and we volumetrically render a feature image, $F_{NR}$ from the given camera. The raw image, $I_{NR}$, is taken to be the first three channels of $F_{NR}$.

\begin{equation}
    \hat{I}_{NR}, F_{NR} = G_{R}(F_{planes}, Rt, K)
\end{equation}

Finally, the superresolution image, $I_{SR}$ is produced by the superresolution module from the raw rendering and feature image. The convolutional layers in $G_{SR}$ are modulated by $w$.

\begin{equation}
    \hat{I}_{SR} = G_{SR}(\hat{I}_{NR}, F_{NR}, w)
\end{equation}

In using dual-discrimination, our discriminator, $D$, takes as input both the superresolution image $\hat{I}_{SR}$ as well as the raw neural rendering $\hat{I}_{NR}$, or the full-resolution image, $I_{SR}$, as well as a downsized copy, $I_{NR}$, when operating on real images. We additionally condition the discriminator on the camera parameters for the given image. Note that R1 regularization is calculated with respect to both $I_{SR}$ and $I_{NR}$.

Our optimization objective is given as the following:

\begin{multline}
    \mathcal{L}(G, D) = \mathbb{E}_{z\sim p_z, Rt\sim p_{Rt}, K\sim p_{K}}[f(D(G(z, Rt, K), Rt, K)] \\
    + \mathbb{E}_{(I_{SR}, I_{NR}, Rt, K) \sim p_{I}} [f(-D(I_{SR}, I_{NR}, Rt, K) \\
    + \gamma ||\nabla_{I_{SR}, I_{NR}} D(I_{SR}, I_{NR}, Rt, K)]||^2 ) ]
\end{multline}

\textcolor{red}{GW: what about the pose conditioning of the discriminator?} 

\textcolor{red}{Due to the limited page count of this manuscript, we include detailed descriptions of the proposed network architecture and training details in the supplement. Source code and pre-trained models will be publicly released.} 

\endinput

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Modelling Pose-Correlated Attribute Distributions \textcolor{red}{GW: still need to edit this}}

In training a 3D-aware model, our goal is to match the distribution of training images while decoupling the effects of appearance and viewpoint. The classic approach to 3D-aware image generation with GANs— to randomly generate scenes while independently sampling camera poses— makes an assumption that the distributions of pose and appearance are independent. While this assumption holds for synthetically generated datasets, it is incorrect for a real-world dataset such as FFHQ. Figure X shows that expression is correlated with camera pitch. As it turns out, people photographed from above are more likely to be smiling than people photographed from below. Additional, more subtle correlations are likely to exist in the dataset. Perhaps, people wearing neckties are more likely to be photographed from steep angles, or people with glasses are never photographed from head-on. While it’s impossible for us to quantify the correlation for every factor, assuming appearance to be completely independent from pose is clearly not the right solution.

Previous attempts at 3D-aware synthesis have fallen into two camps. Some [pi-GAN, GRAF, Lifting?] have assumed appearance and pose to be independent. While such an assumption leads to a high degree of view-consistency, it prevents the model from matching the true, correlated dataset distribution. Consequently, image quality suffers and such methods fail to accurately reproduce the true dataset distribution. Others (HoloGAN, GIRAFFE) rely on network components that are view-inconsistent, which prevent such models from maintaining consistent identity under changing pose. While view-inconsistency allows for synthesized appearance to depend on pose, which lets such models better reflect the correlated distribution, it also makes it difficult to maintain appearance consistency at inference under different viewpoints. The same scene, when rendered from different angles, might experience subtle identity shift; for example, facial expressions might change when moving the camera. While these methods are better at modeling the correlated distributions of appearance and pose, they tend to be less effective at decoupling appearance and pose at inference.


With our approach, we strive for the best of both worlds— we want to allow our model to accurately reflect the dataset distribution, even when viewpoint and appearance are correlated, but we want a way to decouple viewpoint and appearance at inference in order to enable view-consistent rendering. We propose a solution in two parts. With dual-discrimination, we prevent difficult-to-control view-inconsistency and with generator pose conditioning we allow a pathway to modeling a correlated distribution.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Generator Pose Conditioning.} Although dual-discrimination preserves view-consistency, it also prevents the model from learning correlations between appearance and pose. \textcolor{blue}{MC: we still have no evidence for pose-appearance bias. perhaps we could add a small table/figure of "smiliness" by stddevs from the mean angle or other metric? (I have the numbers)} We resolve this shortcoming by offering the generator a pathway for learning an appearance-pose correlated relationship, but a pathway that we can control at inference to decouple appearance and pose. During training, we condition the generator on the target viewpoint. Such conditioning allows the viewpoint to influence scene appearance; for example, a generator conditioned on a pose from above may be more likely to generate a smiling face than a frowning face, in order to better match the dataset distribution. Importantly, this strategy allows us to decouple the effects of appearance and viewpoint at inference. At inference, we can fix the conditioning vector while moving the camera for view-consistent renderings. Alternatively, by fixing the camera while moving the conditioning vector, we reveal the pose-appearance bias present in the dataset. In practice, always conditioning on the true target viewpoint leads to a degenerate solution in which the model produces a “billboard” angled towards the known target viewpoint. We regulate this undesirable effect by randomly swapping the conditioning viewpoint with another random viewpoint with probability p, which is decayed from 1 at the beginning of training.

\ec{Talk about how GPC is a generalization of view-dependent effects. Differentiate ourselves from StyleNeRF/CIPS3D, which simply remove view-dependent effects.}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

